Neutron charge form factor at large $q^2$

The neutron charge form factor $G_{En}(q)$ is determined from an analysis of the deuteron quadrupole form factor $F_{C2}$ data. Recent calculations, based on a variety of different model interactions and currents, indicate that the contributions associated with the uncertain two-body operators of shorter range are relatively small for $F_{C2}$, even at large momentum transfer $q$. Hence, $G_{En}(q)$ can be extracted from $F_{C2}$ at large $q^2$ without undue systematic uncertainties from theory.

==> gen.bbl.tex <==
\begin{thebibliography}{10}

\bibitem{Platchkov90}
S.~Platchkov {\em et al.}
\newblock {\em Nucl. Phys. A}, 510:740, 1990.
\vspace*{-2mm}
          
\bibitem{Galster71}
S.~Galster {\em et al.}
\newblock {\em Nucl. Phys. B}, 32:221, 1971.
\vspace*{-2mm}
          
\bibitem{Meyerhoff94a}
M.~Meyerhoff {\it et al.}
\newblock {\em Phys. Lett. B}, 327:201, 1994.
\vspace*{-2mm}
          
\bibitem{Becker97}
J.~Becker.
\newblock {\em thesis, University of Mainz}, 1997.
\vspace*{-2mm}
          
\bibitem{Becker99}
J.~Becker {\em et al.}
\newblock {\em Eur. Phys. J. A}, 6:329, 1999.
\vspace*{-2mm}
          
\bibitem{Rohe99}
D.~Rohe {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 83:4257, 1999.
\vspace*{-2mm}
          
\bibitem{Herberg99}
C.~Herberg {\em et al.}
\newblock {\em Eur. Phys. J. A}, 5:131, 1999.
\vspace*{-2mm}
          
\bibitem{Eden94}
T.~Eden {\em et al.}
\newblock {\em Phys. Rev. C}, 50:R1749, 1994.
\vspace*{-2mm}
          
\bibitem{Ostrick99}
M.~Ostrick {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 83:276, 1999.
\vspace*{-2mm}
          
\bibitem{Passchier99}
I.~Passchier {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 82:4988, 1999.
\vspace*{-2mm}
          
\bibitem{Ahmidouch01}
A.~Ahmidouch {\em et al.}
\newblock {\em submitted to Phys. Rev. Lett.}
\vspace*{-2mm}
          
\bibitem{Day93x}
D.~Day (spokesperson).
\newblock {\em JLAB experiment E-93-026}.
\vspace*{-2mm}
          
\bibitem{Madey93x}
R.~Madey, B.~Anderson, and S.~Kowalski (spokespersons).
\newblock {\em JLAB experiment E-93-038}.
\vspace*{-2mm}
          
\bibitem{Wiringa95}
R.B. Wiringa, V.G.J. Stoks, and R.~Schiavilla.
\newblock {\em Phys. Rev. C}, 51:38, 1995.
\vspace*{-2mm}
          
\bibitem{Machleidt96}
R.~Machleidt, F.~Sammarruca, and Y.~Song.
\newblock {\em Phys. Rev. C}, 53:1483, 1996.
\vspace*{-2mm}
          
\bibitem{Friar77}
J.~Friar.
\newblock {\em Ann. Phys.}, 104:380, 1977.
\vspace*{-2mm}
          
\bibitem{Forest00}
J.L. Forest.
\newblock {\em Phys. Rev. C}, 61:034007, 2000.
\vspace*{-2mm}
          
\bibitem{Schiavilla01}
R.~Schiavilla.
\newblock {\em Nucl. Phys. A, in print}, 2001.
\vspace*{-2mm}
          
\bibitem{Abbott99}
D.~Abbott {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 82:1379, 1999.
\vspace*{-2mm}
          
\bibitem{Alexa99}
L.C.~Alexa {\em et al}.
\newblock {\em Phys. Rev. Lett.}, 82:1374, 1999.
\vspace*{-2mm}
          
\bibitem{Akimov79}
Yu.K.~Akimov {\em et al.}
\newblock {\em Sov. J. Nucl. Phys.}, 29:335, 1979.
\vspace*{-2mm}
          
\bibitem{Arnold75}
R.G. Arnold {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 35:776, 1975.
\vspace*{-2mm}
          
\bibitem{Arnold87}
R.G. Arnold {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 58:1723, 1987.
\vspace*{-2mm}
          
\bibitem{Auffret85a}
S.~Auffret {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 54:649, 1985.
\vspace*{-2mm}
          
\bibitem{Benaksas66}
D.~Benaksas, D.~Drickey, and D.~Frerejacque.
\newblock {\em Phys. Rev.}, 148:1327, 1966.
\vspace*{-2mm}
          
\bibitem{Berard73a}
R.W. Berard {\em et al.}
\newblock {\em Phys. Lett. B}, 47:355, 1973.
\vspace*{-2mm}
          
\bibitem{Bosted90}
P.E. Bosted {\em et al.}
\newblock {\em Phys. Rev. C}, 42:38, 1990.
\vspace*{-2mm}
          
\bibitem{Bumiller70}
F.A. Bumiller, F.R. Buskirk, J.W. Stewart, and E.B. Dally.
\newblock {\em Phys. Rev. Lett.}, 25:1774, 1970.
\vspace*{-2mm}
          
\bibitem{Buchanan65}
C.D. Buchanan and M.R. Yearian.
\newblock {\em Phys. Rev. Lett.}, 15:303, 1965.
\vspace*{-2mm}
          
\bibitem{Cramer85}
R.~Cramer {\em et al.}
\newblock {\em Z. Phys. C}, 29:513, 1985.
\vspace*{-2mm}
          
\bibitem{Drickey62}
D.~Drickey and L.N. Hand.
\newblock {\em Phys. Rev. Lett.}, 9:521, 1962.
\vspace*{-2mm}
          
\bibitem{Elias69}
J.E. Elias {\em et al.}
\newblock {\em Phys. Rev.}, 177:2075, 1969.
\vspace*{-2mm}
          
\bibitem{Friedman60}
J.I. Friedman, H.W. Kendall, and P.A.M. Gram.
\newblock {\em Phys. Rev.}, 120:992, 1960.
\vspace*{-2mm}
          
\bibitem{Ganichot72}
D.~Ganichot, B.~Grosset\^ete, and D.B. Isabelle.
\newblock {\em Nucl. Phys. A}, 178:545, 1972.
\vspace*{-2mm}
          
\bibitem{Goldemberg64}
J.~Goldemberg and C.~Schaerf.
\newblock {\em Phys. Rev. Lett.}, 12:298, 1964.
\vspace*{-2mm}
          
\bibitem{Honegger97}
A.~Honegger.
\newblock {\em Thesis, Univ. of Basel}, 1999.
\vspace*{-2mm}
          
\bibitem{Grossetete66b}
B.~Grosset\^ete, D.~Drickey, and P.~Lehmann.
\newblock {\em Phys. Rev.}, 141:1425, 1966.
\vspace*{-2mm}
          
\bibitem{Martin77}
F.~Martin {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 38:1320, 1977.
\vspace*{-2mm}
          
\bibitem{Rand67}
R.E. Rand, R.F. Frosch, C.E. Littig, and M.R. Yearian.
\newblock {\em Phys. Rev. Lett.}, 18:469, 1967.
\vspace*{-2mm}
          
\bibitem{Simon81}
G.G. Simon, Ch. Schmitt, and V.H. Walther.
\newblock {\em Nucl. Phys. A}, 364:285, 1981.
\vspace*{-2mm}
          
\bibitem{Stein66}
P.~Stein {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 16:592, 1966.
\vspace*{-2mm}
          
\bibitem{Voitsekhovskii86}
B.B. Voitsekhovskii {\em et al.}
\newblock {\em Pis'ma Zh. Eksp. Teor. Fiz.}, 43:567, 1986.
\vspace*{-2mm}
          
\bibitem{Sick74}
I.~Sick.
\newblock {\em Nucl. Phys. A}, 218:509, 1974.
\vspace*{-2mm}
          
\bibitem{Buchmann96}
A.~Buchmann, H.~Henning, and P.U. Sauer.
\newblock {\em Few Body Syst.}, 21:149, 1996.
\vspace*{-2mm}
          
\bibitem{Henning97}
H.~Henning.
\newblock {\em priv.com.}, 1997.
\vspace*{-2mm}
          
\bibitem{Forest01}
J.L. Forest and R.~Schiavilla.
\newblock {\em to be publ.}
\vspace*{-2mm}
          
\bibitem{Arenhoevel00}
H.~Arenh{\"o}vel, F.~Ritz, and T.~Wilbois.
\newblock {\em Phys. Rev. C}, 61:034002, 2000.
\vspace*{-2mm}
          
\bibitem{VanOrden95}
J.W. VanOrden, N.~Devine, and F.~Gross.
\newblock {\em Phys. Rev. Lett.}, 75:4369, 1995.
\vspace*{-2mm}
          
\bibitem{Hoehler76}
G.~Hoehler {\em et al.}
\newblock {\em Nucl. Phys. B}, 114:505, 1976.
\vspace*{-2mm}
          
\bibitem{Jones00}
M.K.~Jones {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 84:1398, 2000.
\vspace*{-2mm}
          
\bibitem{Popischil00}
Th.~Popischill {\em et al.}
\newblock {\em Eur. Phys. J. C}, to be publ.
\vspace*{-2mm}
          
\bibitem{Milbrath98}
B.D. Milbrath {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 80:452, 1998.
\vspace*{-2mm}
          
\bibitem{Sick01}
I.~Sick.
\newblock {\em Prog. Part. Nucl. Phys., in print}.
\vspace*{-2mm}
          
\bibitem{Arenhoevel01}
H.~Arenh{\"o}vel.
\newblock {\em priv. com.}, 2001.
\vspace*{-2mm}
          
\bibitem{Lung93}
A.~Lung {\em et al.}
\newblock {\em Phys. Rev. Lett.}, 70:718, 1993.
\vspace*{-2mm}
          
      
\end{thebibliography}

